Parity Games on Temporal Graphs

Temporal graphs are a popular modelling mechanism for dynamic complex systems that extend ordinary graphs with discrete time. Simply put, time progresses one unit per step and the availability of edges can change with time. We consider the complexity of solving $\omega$-regular games played on temporal graphs where the edge availability is ultimately periodic and fixed a priori. We show that solving parity games on temporal graphs is decidable in PSPACE, only assuming the edge predicate itself is in PSPACE. A matching lower bound already holds for what we call punctual reachability games on static graphs, where one player wants to reach the target at a given, binary encoded, point in time. We further study syntactic restrictions that imply more efficient procedures. In particular, if the edge predicate is in $P$ and is monotonically increasing for one player and decreasing for the other, then the complexity of solving games is only polynomially increased compared to static graphs.

==> upperbounds.tex <==
\begin{lem}
	Computing the attractor set for $\mathbb{S}$ can be done in PTIME
\end{lem}
\begin{proof}
	Attractor set computation for $\mathbb{S}$, written as $Attr(\mathbb{S})$, allows a relaxation of the rules of an instance of $\mathbb{S}\leq T$. This relaxation allows a vertex to be counted as accepting as soon as it reaches some $v_f\in F$ regardless of whether other possible paths at this timestep are accepting or not. Such behaviour can also be achieved by making every accepting vertex into a reachability player vertex, and adding a reflexive edge to all of them. With this relaxation of the rules, an attractor set $Attr$ can be built in a runtime linear to the amount of vertices $|V|$ within $\mathbb{S}$. This attractor set would also track how many steps it took for some vertex to reach an accepting one. Supposing $v_0$ is the starting vertex, it would then be possible to see if $v_0$ reached an accepting vertex in $T$ or less steps. This can be done in PTIME.
\end{proof}

\begin{lem}
	$\mathbb{S}=T$ is PSPACE-complete
\end{lem}
\begin{proof}
	An algorithm similar to attractor set computation can be used to solve $\mathbb{S}=T$, however the restrictions of this decision problem must be considered. $Attr(\mathbb{S})$ is satisfied if there exists any play that consists of any $T'\leq T$ transitions, where the play consistent with reachability and safety player strategies and results in reaching any accepting vertex $q_f\in F$. $\mathbb{S}=T$ asserts that exactly $T$ rounds must take place in $\mathbb{S}$, so the attractor set computation must be calculated for all such rounds. This can be represented as an inductive set sequence where $0<i\leq T$:
	
	\[Attr_T:=F\]
	\[Attr_{i-1}:=\{v\in V_0: succ(v)\cap Attr_i\}\cup\{v\in V_1: succ(v)\subseteq Attr_i\}\]
	
	Observe how in this sequence of inductive sets, $Attr_i$ will only contain vertices that can reach $q_f\in F$ in exactly $T-i$ steps. After $T$ rounds, $Attr_0$ shall be checked to see if starting vertex $q_0\in Attr_0$. If this is the case, then the reachability player wins in $\mathbb{S}$. As this takes $T$ iterations, the runtime of the algorithm is exponential to the amount of bits needed to represent $T$. If $|V|$ are the amount of vertices in $G$, only $2\cdot|V|$ bits are needed to track the $Attr$ inductive set sequence. This proves PSPACE membership of $\mathbb{S}=T$, and combined with \emph{Lemma 3} proves PSPACE-completeness.
\end{proof}

\begin{lem}
	$\mathbb{T}=T$ is PSPACE-complete if $x\in\mathbb{N},x\in\lambda(e\in E)$ takes constant time to calculate
\end{lem}
\begin{proof}
	Like with how $\mathbb{S}=T$ and $\mathbb{S}\leq T$ were calculated, an algorithm solving $\mathbb{T}=T$ would do so by generating a temporal attractor set. The temporal attractor set computation is similar to the static variant, however $\lambda$ must be considered at every iteration. Let $\lambda succ(v,i)=\{w: (v,w)\in E\land\ i\in\lambda(v,w)\}$. The inductive set of the temporal attractor is also modified, becoming the following:
	
	\[\lambda Attr_T:=F\]
	\[\lambda Attr_{i-1}:=\{v\in V_0: \lambda succ(v,i-1)\cap\lambda Attr_i\}\cup\{v\in V_1: \lambda succ(v)\subseteq \lambda Attr_i\}\]
	
	Due to $\lambda$ needing to be considered at every timestep, it is not possible to compute a temporal attractor in $|Q|$ iterations. $\mathbb{T}\leq T$ may terminate in some $T'\leq T$ iterations, as it can be checked after every round if starting vertex $v_0\in\lambda Attr_i$. It could however at a worst case take $T$ iterations. In particular for $\mathbb{T}=T$, $v_0\in \lambda Attr_0$ must be checked. This takes no more extra space when compared to $\mathbb{S}=T$, and only takes $T$ more operations. Therefore, $\mathbb{T}=T$ is a member of PSPACE and with \emph{Lemma 3} shows PSPACE-completeness.
\end{proof}

\begin{lem}
	Any instance of $\mathbb{T}\leq T$ can be reduced to an instance of $\mathbb{T}=T$
\end{lem}
\begin{proof}
	Let us analyse an instance of $\mathbb{T}\leq T$. A reduction can be made from this to $\mathbb{T}=T$ by constructing a new $\mathbb{T}'$ from the input game $\mathbb{T}$ in the instance of $\mathbb{T}\leq T$. $\mathbb{T}'$ is near identical to $\mathbb{T}$, with some minor modifications applied to the set $E$ and function $\lambda$ of $\mathbb{T}'$. For every accepting vertex $f\in F$ in $\mathbb{T}'$, let $out(f) = \{(f,f)\}$ and $\lambda(f,f)=\{0,1,\ldots,T-1\}$. This transforms every accepting vertex in $\mathbb{T}'$ into sink vertices, guaranteeing that if they are visited before some timestep $T'\leq T$, they will be available at $T$ too. Let $WIN(\mathbb{T})$ be the set of starting vertices from which the reachability player wins in $\mathbb{T}$ depending on the specific decision problem. If $\mathbb{T}'$ is constructed in the way defined above, then $WIN(\mathbb{T})=WIN(\mathbb{T}')$. 
\end{proof}

\begin{cor}
	$\mathbb{T}\leq T$ is PSPACE-complete if $x\in\mathbb{N},x\in\lambda(e\in E)$ takes constant time to calculate
\end{cor}

\begin{lem}
	Encoding $\lambda$ using Presburger arithmetic with no restrictions would increase computational complexity of $\mathbb{T}=T$, whereas existential Presburger would not
\end{lem}
\begin{proof}
	If $\lambda$ is encoded as a naive subset or as intervals of integers, then $x\in\mathbb{N},x\in\lambda(e\in E)$ will discover edge membership at a given timestep $x$ in a constant amount of operations. However, such a representation may not be nuanced enough to capture the exact set of timesteps that it is desired edges be active for. This would lead us to look for more nuanced representations, such as semilinear sets.  These types of sets have a property that is known as being `ultimately periodic': Although initially the set may not seem to have some kind of linear progression, eventually there will be some defined point from which the rest of the set progression will be linear. All such semilinear sets can be defined through usage of Presburger arithmetic. With no restrictions, deriving a semilinear set from a first order logic statement utilising Presburger arithmetic may take a doubly exponential amount of time, with an upper bound itself of being triply exponential. An example of using Presburger arithmetic to encode a statement representing the semilinear set of $\{1,2,3,4\}\cup\{x: y\in\mathbb{N}\land x=2y+1\}$ would look something like:
	\[\varphi:=\forall x.\exists y.((y=(x+(x+1)))\lor(y=1)\lor(y=(1+1))\lor(y=(1+(1+1)))\]
	\[\lor(y=(1+(1+(1+1)))))\]
	Although the Presburger statement is more verbose than the initial representation of the semilinear set, it is actually decidable unlike said initial representation which uses Peano axioms. Considering that $x\in\mathbb{N},x\in\lambda(e\in E)$ would have to be re-calculated for every single iteration of calculating $\mathbb{T}=T$ or $\mathbb{T}\leq T$, this could result in hypothetically a $T$ amount of triply exponential Presburger arithmetic calculation operations being invoked.
	
	Suppose that the following restriction is imposed on the Presburger arithmetic used: universal quantifier $\forall$ is forbidden. A problem requiring existential Presburger formulae to be derived into a semilinear set using quantifier elimination is NP-Complete. If this existential Presburger was used to encode $\lambda$ instead, then the complexity of $\mathbb{T}=T$ would remain PSPACE-complete.
\end{proof}

\begin{cor}
	Encoding $\lambda$ using Presburger arithmetic with no restrictions would increase computational complexity of $\mathbb{T}\leq T$, whereas existential Presburger would not
\end{cor}
